Let-It-Flow: Simultaneous Optimization of 3D Flow and Object Clustering

We study the problem of self-supervised 3D scene flow estimation from real large-scale raw point cloud sequences, which is crucial to various tasks like trajectory prediction or instance segmentation. In the absence of ground truth scene flow labels, contemporary approaches concentrate on deducing optimizing flow across sequential pairs of point clouds by incorporating structure based regularization on flow and object rigidity. The rigid objects are estimated by a variety of 3D spatial clustering methods. While state-of-the-art methods successfully capture overall scene motion using the Neural Prior structure, they encounter challenges in discerning multi-object motions. We identified the structural constraints and the use of large and strict rigid clusters as the main pitfall of the current approaches and we propose a novel clustering approach that allows for combination of overlapping soft clusters as well as non-overlapping rigid clusters representation. Flow is then jointly estimated with progressively growing non-overlapping rigid clusters together with fixed size overlapping soft clusters. We evaluate our method on multiple datasets with LiDAR point clouds, demonstrating the superior performance over the self-supervised baselines reaching new state of the art results. Our method especially excels in resolving flow in complicated dynamic scenes with multiple independently moving objects close to each other which includes pedestrians, cyclists and other vulnerable road users. Our codes are publicly available on https://github.com/ctu-vras/let-it-flow.

==> preamble.tex <==
%
% --- inline annotations
%
% \usepackage[dvipsnames]{xcolor}
% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/revision.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\linewidth]{img/speed_performance.png}
%     \caption{Speed performance comparison between~\cite{Li2023Fast,li2021neural,vidanapathirana2023mbnsf}}
    
    % \label{fig:speed}
% \end{figure}
% 
\begin{tikzpicture}
    \draw (0, 0) node[inner sep=0]{
    \centering \includegraphics[width=0.99\linewidth]{img/speed_performance.png}}
    ;
    \draw (3., 2.11) node {\cite{Li2023Fast}};
    \draw (3., 1.71) node {\cite{li2021neural}};
    \draw (3., 1.31) node {\cite{vidanapathirana2023mbnsf}};
\end{tikzpicture}
\captionof{figure}{Speed performance comparison between the optimization-based methods with Neural Prior regularizer. We show ratio between the performance and time spent of iterations. The Fast Neural Prior~\cite{Li2023Fast} converges fastest and Our proposed loss achieves the best performance. All measured with accelerator proposed in~\cite{Li2023Fast}.}
\label{fig:speed}

\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.99\linewidth]{img/dbscan_and_knn.png}
    \includegraphics[width=0.99\linewidth]{img/both_clusters.png}
    \caption{\textbf{On the left} - clusters from method \cite{vidanapathirana2023mbnsf}, where each color denotes a single DBSCAN cluster meant for a single rigid motion fit with outlier rejection. \textbf{On the right} - our over-segmentation Euclidean clustering (each cluster denoted by color) and soft rigidity connections that can overflow into more objects but can be rejected as outliers. We observe that a building with three pedestrians clustered can only allow for a single rigid motion (stationary from more building points) and reject the pedestrian motion in the loss for the previous method. On the other hand, motions on the right are treated separately for each object, with the exception of two pedestrians walking right next to each other in the same direction and a few noisy points not predicted by ground removal.}
    \label{fig:clusters}
\end{figure*}
% 
% 
\subsection{Reviewer: 1}
% 
% Weakness:
\textbf{Question 1:} The authors claim that the main novelty of this method is replacing the original clustering method, DBSCAN, with two types of clusters: hard rigid clusters and soft rigid clusters (Line 44, Page 2).
However, as shown in the "Implementation Details" (Page 5), the hard rigid clusters are still obtained using DBSCAN. The soft rigid clusters are generated by the soft rigidity loss, which is very similar to the Multi-Body Regularization proposed in~\cite{vidanapathirana2023mbnsf}.
Thus, this method's novelty is incremental.

\textbf{Answer:} We used the DBSCAN method only as an implementation of grouping the points within the Euclidean distance lower than 0.3 meters as a tool for over-segmentation. As we used these parameters and allowed for single point clusters, the usage of DBSCAN is equal to connecting points with a distance lower than 0.3 meters. We agree that the wording is confusing, and we now refer to it correctly as an \textbf{Euclidean Clustering}. Specifically, if the Euclidean distance of two points is smaller than 0.3m, they are assigned to the same cluster. Otherwise, they are not.

Regarding the novelty, our method allows for flow estimation on smaller objects, see Figure 4. in our submission, whereas the~\cite{vidanapathirana2023mbnsf} does not due to the following reasons: 
\begin{itemize}
    \item ~\cite{vidanapathirana2023mbnsf} relies on large DBSCAN clusters (0.8 meters grouping radius and condition of at least 30 points in cluster to be considered valid) that merge small and large close objects together and enforce single rigid motion for them. The proposed soft rigidity is able to group points and reject interconnections between the overlapping clusters; see attached Figure~\ref{fig:clusters}.
    \item Our spatial-temporal hard cluster over-segmentation allows for leveraging adjacent measurements for clustering, unlike the~\cite{vidanapathirana2023mbnsf} single frame DBSCAN. 
    \item We also compute rigidity on all points as we over-segment all samples, whereas~\cite{vidanapathirana2023mbnsf} consider unclustered (points that do not have at least 30 other points within the radius of 0.8 meters) as noise and do not perform rigidity regularization on them. Such selection greatly reduces the potential of rigidity regularization in greater distances.
    \item Due to the novel overlapping clusters that allows for great parallelization, we simultaneously achieve speed-up and performance boost.
    \item Another big difference is that our method does not rely on Neural prior implicit flow field regularizer as~\cite{vidanapathirana2023mbnsf}, but on these over-lapping clusters instead. Such design significantly helps in Pedestrian and Cyclist flow estimation as low point objects do not contribute to the final loss significantly in baseline~\cite{vidanapathirana2023mbnsf}, whereas our over-segmentation clusters and over-lapping clusters allows for independent optimization of flows per objects. See Table II in submission paper for the difference.
\end{itemize}

% The aforementioned reasons highlight the practical differences


\textbf{Question 2:} As presented in Table V, only a very slight improvement is observed from merging hard clusters with the guidance of flow. Does this imply that this mechanism is ineffective?

\textbf{Answer:} This submodule of the method connects the clusters over time, forward and backward, which helps in preventing degenerative solutions and helps in reaching the full instance segmentation. As a result, the effect of this mechanism is to refine the speed of objects and catch lonely clusters that can be otherwise regarded as other objects traveling in different directions, which might confuse the detection system. We see it as a practical addition due to the aforementioned reason, and even though the absolute difference value is small, it is non-negligible (2.5\% relative improvement on dynamic \textit{EPE}) to the remaining error.
% Degenerative solutions

\textbf{Question 3:} As presented in Fig. 5, FastNSF~\cite{Li2023Fast} consumes significantly more than 1 second. However, according to the FastNSF paper, it is reported to be below 1 second.


\textbf{Answer:} We apologize for confusion in speed evaluation, it was not intended. The final position of~\cite{Li2023Fast} in Figure 5 in submission paper comes from the fixed number of iterations that empirically led Neural Prior architecture to convergence. However, we did not use the same convergence criterion (value of loss difference between iterations) as in~\cite{Li2023Fast} to stop optimization sooner, as we focused on~\cite{vidanapathirana2023mbnsf} comparison (we did not even describe the speed comparison within~\cite{Li2023Fast} in the text) where the final number of iterations are bigger. 
The method~\cite{Li2023Fast}, in fact, does converge sooner, and we updated Figure~\ref{fig:speed} with the full iteration path of \cite{Li2023Fast} to complete the picture. The interpretation is indeed that \cite{Li2023Fast} converges sooner than our method, but with a worse final performance.



\subsection{Reviewer: 2}

\textbf{Question 1:} The method is called self-supervised but it is seems a direct optimization method.

\textbf{Answer:} Good point; we changed it to optimization. We used the word self-supervised to express that the method falls into the family of methods without the need for supervision.

\textbf{Question 2:} Divide and merge clustering is not new. Here, only merge is being used (Agglomerative clustering and DBSCAN are examples). There are bottom up and top down such methods. The proposed method has some novelty in the use case of scene flow and the way it controls the merge during the joint optimization, but a better connection to other similar ideas would be beneficial.

\textbf{Answer:} We agree and we upgraded the related work section with such methods. Namely Agglomerative Clustering~\cite{Zepeda-Mendoza2013}, HDBSCAN~\cite{hdbscan}, WardLinkage~\cite{Ward1963HierarchicalGT}, BIRCH~\cite{birch}. All methods use either hard clustering or hierarchical structures as a final output. They do not use overlapping clusters and flow guidance like our method.
% 

\textbf{Question 3:} Figure 1 is hard to follow in a first glance (but is well explained in the text). Please consider adding a reference to the text in the caption.

\textbf{Answer:} Added reference.

\textbf{Question 4:} The algorithm: step 3): how the minimization is applied? it is not mentioned in the text and it is not clear. Since this is an iterative method with many local minimum, how the flow is initialized?

\textbf{Answer:} The flow is initialized as a zero vector, and minimization is applied as a gradient optimization to minimize the final loss function with the Adam optimizer. Thanks for pinpointing this. We have included this in the revision. The reason for initialization in zero is that it is likely that the nearest neighbor is going to be the same object next time (after ICP ego-motion compensation).

\textbf{Question 5:} equation 2: if $r_{ij}$ should lie in [0,1], theta cannot be fixed. The text said it is. Not clear to me.

\textbf{Answer:} Thank you for your very valuable comment. This is a boundary condition that is never exceeded during the optimization process due to the initialization of flow in zero. The loss itself prevents numerically unstable cases (such as flow split on a single object into multiple directions). That being said, we added clipping of the values to prevent potential numerical instability, as you mentioned, and we add a description of clipping into equation 2.


\textbf{Question 6:} What is the learning rate, mentioned only in pp. 5 line 22. if it is related to the minimization, it should be explained.

\textbf{Answer:} Thank you for catching the incompleteness. It is a learning rate related to minimization (performed by the Adam optimizer). We added the information.

\textbf{Question 7:} Outlier detection and removal: this is mentioned in the text, but there is no explanation of how this is done. how points are removed or disregarded? the text only says that theta controls this, but nothing else.

\textbf{Answer:} The final soft loss is weighted by the score from the eigenvalues of $\mathbf{A}_m$. As a result, this weighting automatically decreases the effect of loss on outlier points by multiplication with smaller values. It is not hard outlier rejection, but soft decided by the algorithm. We have highlighted it in the text.


\textbf{Question 8:} pp. 6, DBSCAN: in the implementation section it says that parameter 0.3 is being used but in this section, it says that a new approach is designed for over segmentation. Do all experiments use the same method/parameter?

\textbf{Answer:} Yes, all experiments use the same parameters. We empirically chose this value based on observation of a few frames and the idea that objects move with some space around them, and we modeled it with this number. This value is related mainly to the size of objects and sparsity of the sensor.

\textbf{Question 9:} Would be interesting to test how clustering parameters/setup affect the results because it's expected to be quite sensitive to this initialization and the method does not divide clusters, just merges.

\textbf{Answer:} We run the ablation study for your proposal in Figure~\ref{fig:eps-plot}. The hard clustering parameter Epsilon which denotes the grouping radius for Euclidean clustering. If the parameter is zero (no points are considered rigid in hard clusters), we see a decrease in dynamic EPE, as the flows are inconsistent on object structures. The higher we set the epsilon, the clusters with multiple objects emerge. When we perform Euclidean clustering with accumulated point clouds in adjacent frames, we observe values around 0.2 to bring the best performance. Note that soft-clustering (defined by fixed number of nearest neighbors for clusters) is included in the experiment and we just ablate the hard clustering part.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{img/clustering_plot.png}
    \caption{The hard clustering parameter Epsilon which denotes the grouping radius for Euclidean clustering compared to dynamic end-point-error.}
    \label{fig:eps-plot}
\end{figure}

\textbf{Question 10:} Clustering: since divide and merge methods are not new, I would add more references to these and try to connect them to the proposed method. 

\textbf{Answer:} Thank you for the recommendation, we added the clustering related methods. 


